CaT-BENCH: Benchmarking Language Model Understanding of Causal and Temporal Dependencies in Plans

Understanding the abilities of LLMs to reason about natural language plans, such as instructional text and recipes, is critical to reliably using them in decision-making systems. A fundamental aspect of plans is the temporal order in which their steps needs to be executed, which reflects the underlying causal dependencies between them. We introduce CaT-Bench, a benchmark of Step Order Prediction questions, which test whether a step must necessarily occur before or after another in cooking recipe plans. We use this to evaluate how well frontier LLMs understand causal and temporal dependencies. We find that SOTA LLMs are underwhelming (best zero-shot is only 0.59 in F1), and are biased towards predicting dependence more often, perhaps relying on temporal order of steps as a heuristic. While prompting for explanations and using few-shot examples improve performance, the best F1 result is only 0.73. Further, human evaluation of explanations along with answer correctness show that, on average, humans do not agree with model reasoning. Surprisingly, we also find that explaining after answering leads to better performance than normal chain-of-thought prompting, and LLM answers are not consistent across questions about the same step pairs. Overall, results show that LLMs' ability to detect dependence between steps has significant room for improvement.

==> figs/before_after_fig.tex <==
\begin{figure*}[!tbh]
\centering
\begin{subfigure}[t]{\columnwidth}
  \includegraphics[width=\columnwidth]{figs/before_after_binary.png}
  \caption{Models just predicting the dependency (P)}
  \label{fig:before_after_binary} 
\end{subfigure}
\begin{subfigure}[t]{\columnwidth}
  \includegraphics[width=\columnwidth]{figs/before_after_binary_expl.png}
  \caption{Models predicting the dependency and explaining the prediction (P$\rightarrow$E)}
  \label{fig:before_after_binary_expl}
\end{subfigure}
\caption{Performance of models in different settings on the \binarytask~ task split by the type of temporal relation (\textit{before} and \textit{after}) asked about in the question.\yash{f1 for before, f1 for affter and \tc}}
\label{fig:before_after}
\end{figure*}

==> figs/far_close_fig.tex <==
\begin{figure*}[!tbh]
\centering
\begin{subfigure}[t]{\columnwidth}
  \includegraphics[width=\columnwidth]{figs/far_close_binary.png}
  \caption{Models just predicting the dependency (P)}
  \label{fig:far_close_binary} 
\end{subfigure}
\begin{subfigure}[t]{\columnwidth}
  \includegraphics[width=\columnwidth]{figs/far_close_binary_expl.png}
  \caption{Models predicting the dependency and explaining the prediction (P$\rightarrow$E)}
  \label{fig:far_close_binary_expl}
\end{subfigure}
\caption{Performance of models in different settings on the \binarytask~ task split by the distance between the steps being asked about in the question.\yash{look at f1 of these instead of accuracy, should have more nuance}}
\label{fig:far_close}
\end{figure*}

==> tables/after.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{| l | l | l | l | l |}
\toprule
 & Accuracy & Precision & Recall & F1 \\
\midrule
\gthree (P$\rightarrow$E) & 63.62\% & 0.46 & 0.56 & 0.51 \\
\gthree (P) & 70.47\% & 0.6 & 0.34 & 0.43 \\
\midrule
\gfturbo (P$\rightarrow$E) & 79.86\% & 0.73 & 0.63 & 0.67 \\
\gfturbo (P) & 62.36\% & 0.36 & 0.63 & 0.45 \\
\midrule
\gfomni (P$\rightarrow$E) & 74.32\% & 0.59 & 0.73 & 0.65 \\
\gfomni (P) & 54.32\% & 0.41 & 0.85 & 0.55 \\
\midrule
\llama (P$\rightarrow$E) & 58.92\% & 0.42 & 0.63 & 0.51 \\
\llama (P) & 56.38\% & 0.41 & 0.67 & 0.51 \\
\midrule
\gem (P$\rightarrow$E) & 59.95\% & 0.4 & 0.42 & 0.41 \\
\gem (P) & 67.14\% & 0.51 & 0.26 & 0.35 \\
\midrule
\gemadv (P$\rightarrow$E) & 72.96\% & 0.56 & 0.94 & 0.7 \\
\gemadv (P) & 52.91\% & 0.37 & 0.56 & 0.44 \\
\bottomrule
\end{tabular}
\caption{Performance of different models on questions that ask about the after aspect}
\label{tab:after}
\end{table*}

==> tables/all_human_eval.tex <==
\begin{table}[!ht]
\centering
\begin{tabular}{| l  |r  |r  |r  |}
\toprule
 & \avg & \binavg & \maj \\
\midrule
Llama3 & 3.19 & 0.53 & 53.01\% \\
Turbo & 3.82 & 0.73 & 77.05\% \\
Omni & 3.82 & 0.74 & 78.43\% \\
\bottomrule
\end{tabular}
\caption{Human evaluation metrics for explanations generated by various models.}
\label{tab:all_human}
\end{table}

==> tables/automatic_all_expts.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{| l | c | c | c | c | c | c | c |}
\toprule
Model & Experiment & Acc & P & R & F1 & \tc & \ndsc \\
\midrule
\multirow{2}{*}{\gthree } & (P$\rightarrow$E) & 53.47 & 0.39 & 0.71 & 0.5 & 51.17 & 73.31 \\
 & (P) & 63.43 & 0.46 & 0.50 & 0.48 & 55.31 & 70.42 \\
\midrule
\multirow{2}{*}{\gfturbo} & (P$\rightarrow$E) & 73.26 & 0.57 & 0.79 & 0.66 & 60.89 & 66.97 \\
 & (P) & 59.32 & 0.44 & 0.81 & 0.57 & 47.84 & 70.28 \\
\midrule
\multirow{2}{*}{\gfomni} & (P$\rightarrow$E) & 75.47 & 0.59 & 0.86 & 0.7 & 72.91 & 58.17 \\
 & (P) & 56.60 & 0.43 & 0.92 & 0.59 & 75.92 & 47.96 \\
\midrule
\multirow{2}{*}{\llama} & (P$\rightarrow$E) & 47.02 & 0.37 & 0.82 & 0.51 & 51.69 & 83.38 \\
 & (P) & 45.38 & 0.36 & 0.84 & 0.51 & 56.10 & 83.87 \\
\midrule
\multirow{2}{*}{\gem} & (P$\rightarrow$E) & 57.32 & 0.41 & 0.65 & 0.50 & 53.80 & 66.90 \\
 & (P) & 61.08 & 0.42 & 0.45 & 0.43 & 56.90 & 73.80 \\
\midrule
\multirow{2}{*}{\gemadv} & (P$\rightarrow$E) & 72.00 & 0.55 & 0.93 & 0.69 & 77.89 & 60.21 \\
 & (P) & 54.98 & 0.41 & 0.77 & 0.53 & 59.91 & 58.24 \\
\bottomrule
\end{tabular}
\caption{Performance of all benchmark models on the \binarytask~ task when just making a prediction (P) and when also explaining the prediction (P$\rightarrow$E). 
Acc represents Accuracy, P represents Precision and R denotes Recall metric.
Accuracy, \tc and \ndsc are percentages on a scale of 0-100\% while the others are on a scale of 0-1.
}
\label{tab:auto_eval}
\end{table*}

==> tables/before.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{| l | l | l | l | l |}
\toprule
 & Accuracy & Precision & Recall & F1 \\
\midrule
\gthree (P$\rightarrow$E) & 43.33\% & 0.36 & 0.86 & 0.5 \\
\hline
\gthree (P) & 56.38\% & 0.41 & 0.66 & 0.5 \\
\midrule
\gfturbo (P$\rightarrow$E) & 66.67\% & 0.5 & 0.96 & 0.66 \\
\hline
\gfturbo (P) & 53.24\% & 0.52 & 0.99 & 0.68 \\
\midrule
\gfomni (P$\rightarrow$E) & 76.62\% & 0.59 & 0.99 & 0.74 \\
\hline
\gfomni (P) & 58.87\% & 0.45 & 0.99 & 0.62 \\
\midrule
\llama (P$\rightarrow$E) & 35.12\% & 0.34 & 1 & 0.51 \\
\hline
\llama (P) & 34.37\% & 0.34 & 1 & 0.51 \\
\midrule
\gem (P$\rightarrow$E) & 54.69\% & 0.42 & 0.88 & 0.57 \\
\hline
\gem (P) & 55.02\% & 0.39 & 0.63 & 0.48 \\
\midrule
\gemadv (P$\rightarrow$E) & 71.03\% & 0.54 & 0.92 & 0.68 \\
\hline
\gemadv (P) & 57.04\% & 0.44 & 0.97 & 0.6 \\
\bottomrule
\end{tabular}
\caption{Performance of different models on questions that ask about the before aspect}
\label{tab:before}
\end{table*}

==> tables/close.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{| l | l | l | l | l | l | l |}
\toprule
 & \dep & \ndep & \ndeps & \ours & \tc & \ndsc \\
\midrule
\gthree (P$\rightarrow$E) & 87.27\% & 37.91\% & 38.24\% & 55.03\% & 66.38\% & 70.59\% \\
\gthree (P) & 69.41\% & 66.67\% & 68.63\% & 68.25\% & 63.28\% & 66.01\% \\
\midrule
\gfturbo (P$\rightarrow$E) & 89.44\% & 58.50\% & 77.45\% & 75.37\% & 73.02\% & 67.32\% \\
\gfturbo (P) & 92.39\% & 40.09\% & 51.80\% & 58.88\% & 62.74\% & 70.10\% \\
\midrule
\gfomni (P$\rightarrow$E) & 95.65\% & 52.94\% & 78.76\% & 76.12\% & 81.58\% & 57.19\% \\
\gfomni (P) & 98.60\% & 18.46\% & 51.47\% & 56.91\% & 82.76\% & 52.61\% \\
\midrule
\llama (P$\rightarrow$E) & 98.45\% & 14.38\% & 19.44\% & 45.02\% & 78.91\% & 83.17\% \\
\llama (P) & 97.67\% & 13.40\% & 18.79\% & 44.22\% & 78.37\% & 85.13\% \\
\midrule
\gem (P$\rightarrow$E) & 82.92\% & 39.22\% & 44.77\% & 56.10\% & 62.53\% & 66.99\% \\
\gem (P) & 68.17\% & 55.07\% & 59.48\% & 61.03\% & 55.67\% & 68.14\% \\
\midrule
\gemadv (P$\rightarrow$E) & 95.50\% & 54.58\% & 65.69\% & 72.32\% & 80.19\% & 59.80\% \\
\gemadv (P) & 92.39\% & 37.75\% & 45.59\% & 59.15\% & 72.27\% & 62.42\% \\
\bottomrule
\end{tabular}
\caption{Performance of different models on the Step Order Prediction task when the steps being asked about are close to each other.}
\label{tab:close}
\end{table*}

==> tables/cot_old.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{| l | l | l | l | l | l | l |}
\toprule
 & Accuracy & Precision & Recall & F1 & \tc & \ndsc \\
\midrule
\gfturbo (P$\rightarrow$E) & 73.26\% & 0.57 & 0.79 & 0.66 & 60.89\% & 66.97\% \\
\gfturbo (E$\rightarrow$P) & 61.36\% & 0.46 & 0.98 & 0.63 & 69.06\% & 67.75\% \\
\gfturbo (P) & 59.32\% & 0.44 & 0.81 & 0.57 & 47.84\% & 70.28\% \\
\midrule
\gfomni (P$\rightarrow$E) & 75.47\% & 0.59 & 0.86 & 0.7 & 72.91\% & 58.17\% \\
\gfomni (E$\rightarrow$P) & 61.36\% & 0.46 & 0.98 & 0.63 & 78.97\% & 53.73\% \\
\gfomni (P) & 56.60\% & 0.43 & 0.92 & 0.59 & 75.92\% & 47.96\% \\
\bottomrule
\end{tabular}
\caption{Performance of \gfour models on the Step Order Prediction task when just predicting the dependency vs predicting and then explaining the judgment (P$\rightarrow$E) vs using chain of thought prompting (E$\rightarrow$P).}
\label{tab:binary_explain_vs_cot}
\end{table*}

==> tables/d_human_eval.tex <==
\begin{table}[!tbh]
\centering
\begin{tabular}{| l | r | r | r |}
\toprule
 & \avg & \binavg & \maj \\
\midrule
Llama3 & 3.76 & 0.7 & 75.21\% \\
Turbo & 3.94 & 0.77 & 79.41\% \\
Omni & 4.08 & 0.83 & 87.82\% \\
\bottomrule
\end{tabular}
\caption{Human evaluation metrics for explanations generated by various models for \dep questions}
\label{tab:d_human}
\end{table}


==> tables/d_nd_nds.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{| l | c | c | c | c | c | c |}
\toprule
 & \multicolumn{2}{c|}{\dep} & \multicolumn{2}{c|}{\ndep} & \multicolumn{2}{c|}{\ndeps} \\
\midrule
 & Acc & \tc & Acc & \tc & Acc & \tc \\
\midrule
\gthree (P$\rightarrow$E) & 70.77 & 59.58 & 44.93 & 38.87 & 44.72 & 55.07 \\
\gthree (P) & 50.00 & 54.93 & 69.44 & 49.86 & 70.85 & 61.13 \\
\midrule
\gfturbo (P$\rightarrow$E) & 79.44 & 64.79 & 59.08 & 45.21 & 81.24 & 72.68 \\
\gfturbo (P) & 80.77 & 62.96 & 38.52 & 34.79 & 58.66 & 45.77 \\
\midrule
\gfomni (P$\rightarrow$E) & 85.56 & 72.25 & 56.55 & 56.55 & 84.30 & 84.30 \\
\gfomni (P) & 92.11 & 68.03 & 18.87 & 75.21 & 58.80 & 68.03 \\
\midrule
\llama (P$\rightarrow$E) & 81.62 & 63.24 & 26.41 & 48.31 & 33.03 & 43.52 \\
\llama (P) & 83.66 & 67.32 & 23.38 & 53.52 & 29.08 & 47.46 \\
\midrule
\gem (P$\rightarrow$E) & 64.93 & 49.86 & 49.79 & 49.72 & 57.25 & 61.83 \\
\gem (P) & 44.79 & 56.62 & 66.20 & 50.14 & 72.25 & 63.94 \\
\midrule
\gemadv (P$\rightarrow$E) & 93.10 & 89.58 & 54.44 & 69.72 & 68.45 & 74.37 \\
\gemadv (P) & 76.69 & 57.04 & 36.90 & 53.24 & 51.34 & 69.44 \\
\bottomrule
\end{tabular}
\caption{Accuracy and temporal consistency of different models on the Step Order Prediction Task when split by question types in \ours.
Accuracy and \tc are percentages on a scale of 0-100\%.
\nate{What do you think about adding a majority class baseline and/or random chance row?}
}
\label{tab:d_nd_nds}
\end{table*}

==> tables/far.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{| l | l | l | l | l | l | l |}
\toprule
 & \dep & \ndep & \ndeps & \ours & \tc & \ndsc \\
\midrule
\gthree (P$\rightarrow$E) & 57.09\% & 50.25\% & 49.63\% & 52.26\% & 39.30\% & 75.37\% \\
\gthree (P) & 33.89\% & 71.53\% & 72.52\% & 59.66\% & 49.08\% & 73.76\% \\
\midrule
\gfturbo (P$\rightarrow$E) & 71.13\% & 59.53\% & 84.16\% & 71.61\% & 51.42\% & 66.71\% \\
\gfturbo (P) & 71.13\% & 40.72\% & 63.86\% & 58.40\% & 36.20\% & 70.42\% \\
\midrule
\gfomni (P$\rightarrow$E) & 77.19\% & 59.28\% & 88.49\% & 74.96\% & 66.14\% & 58.91\% \\
\gfomni (P) & 86.73\% & 19.18\% & 64.36\% & 56.35\% & 70.57\% & 44.43\% \\
\midrule
\llama (P$\rightarrow$E) & 67.65\% & 35.52\% & 43.32\% & 48.58\% & 30.43\% & 83.54\% \\
\llama (P) & 72.04\% & 30.94\% & 36.88\% & 46.28\% & 38.71\% & 82.92\% \\
\midrule
\gem (P$\rightarrow$E) & 50\% & 57.80\% & 66.71\% & 58.28\% & 46.99\% & 66.83\% \\
\gem (P) & 25.39\% & 74.63\% & 81.93\% & 61.12\% & 57.86\% & 78.09\% \\
\midrule
\gemadv (P$\rightarrow$E) & 91.11\% & 54.33\% & 70.54\% & 71.74\% & 76.09\% & 60.52\% \\
\gemadv (P) & 63.66\% & 36.26\% & 55.69\% & 51.71\% & 50.25\% & 55.07\% \\
\bottomrule
\end{tabular}
\caption{Performance of different models on the Step Order Prediction task when the steps being asked about are far from each other.}
\label{tab:far}
\end{table*}

==> tables/nd_human_eval.tex <==
\begin{table}[!tbh]
\centering
\begin{tabular}{| l  |r  |r  |r  |}
\toprule
 & \avg & \binavg & \maj \\
\midrule
Llama3 & 2.75 & 0.4 & 35.83\% \\
Turbo & 3.74 & 0.7 & 75.83\% \\
Omni & 3.6 & 0.66 & 71.67\% \\
\bottomrule
\end{tabular}
\caption{Human evaluation metrics for explanations generated by various models for \ndep questions}
\label{tab:nd_human}
\end{table}


==> tables/nds_human_eval.tex <==
\begin{table}[!tbh]
\centering
\begin{tabular}{| l  |l  |l  |l  |l |}
\toprule
 & \avg & \binavg & \maj \\
\midrule
Llama3 & 2.84 & 0.42 & 39.53\% \\
Turbo & 3.68 & 0.67 & 73.24\% \\
Omni & 3.7 & 0.71 & 71.08\% \\
\bottomrule
\end{tabular}
\caption{Human evaluation metrics for explanations generated by various models for \ndeps questions}
\label{tab:nds_human}
\end{table}


==> tables/nds_prf.tex <==
\begin{table}[!tbh]
\centering
\begin{tabular}{| l | l | l | l | l |}
\hline
 &  & \multicolumn{3}{c|}{\ndeps} \\
\hline
 &  & P & R & F \\
\hline
\multirow{2}{*}{\gthree} & (A) & 0.59 & 0.71 & 0.64 \\
 & (A+E) & 0.6 & 0.45 & 0.51 \\
\hline
\multirow{2}{*}{\gfturbo} & (A) & 0.75 & 0.59 & 0.66 \\
 & (A+E) & 0.8 & 0.81 & 0.81 \\
\hline
\multirow{2}{*}{\gfomni} & (A) & 0.88 & 0.59 & 0.71 \\
 & (A+E) & 0.85 & 0.84 & 0.85 \\
\hline
\multirow{2}{*}{\llama} & (A) & 0.64 & 0.29 & 0.4 \\
 & (A+E) & 0.64 & 0.33 & 0.44 \\
\hline
\multirow{2}{*}{\gem} & (A) & 0.57 & 0.72 & 0.64 \\
 & (A+E) & 0.62 & 0.57 & 0.6 \\
\hline
\multirow{2}{*}{\gemadv} & (A) & 0.69 & 0.51 & 0.59 \\
 & (A+E) & 0.91 & 0.68 & 0.78 \\
\hline
\multirow{2}{*}{\flash} & (A) & 0.6 & 0.46 & 0.52 \\
 & (A+E) & 0.65 & 0.48 & 0.55 \\
\hline
\end{tabular}
\caption{Performance of models on \ndeps}
\label{tab:nds_prf}
\end{table}


==> tables/step_order_prediction_results.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{| l | l | l | l | l | l | l |}
\toprule
 & Accuracy & Precision & Recall & F1 & \tc & \ndsc \\
\midrule
\gthree & 63.43\% & 0.46 & 0.5 & 0.48 & 55.31\% & 70.42\% \\
\gfturbo & 59.32\% & 0.44 & 0.81 & 0.57 & 47.84\% & 70.28\% \\
\gfomni & 56.60\% & 0.43 & 0.92 & 0.59 & 75.92\% & 47.96\% \\
\llama & 45.38\% & 0.36 & 0.84 & 0.51 & 56.10\% & 83.87\% \\
\gem & 61.08\% & 0.42 & 0.45 & 0.43 & 56.90\% & 73.80\% \\
\gemadv & 54.98\% & 0.41 & 0.77 & 0.53 & 59.91\% & 58.24\% \\
\bottomrule
\end{tabular}
\caption{Performance of different models on the Step Order Prediction task.}
\label{tab:binary}
\end{table*}


==> tables/step_order_prediction_results_using_explanations.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{| l | l | l | l | l | l | l |}
\toprule
 & Accuracy & Precision & Recall & F1 & \tc & \ndsc \\
\midrule
\gthree & 53.47\% & 0.39 & 0.71 & 0.5 & 51.17\% & 73.31\% \\
\gfturbo & 73.26\% & 0.57 & 0.79 & 0.66 & 60.89\% & 66.97\% \\
\gfomni & 75.47\% & 0.59 & 0.86 & 0.7 & 72.91\% & 58.17\% \\
\llama & 47.02\% & 0.37 & 0.82 & 0.51 & 51.69\% & 83.38\% \\
\gem & 57.32\% & 0.41 & 0.65 & 0.5 & 53.80\% & 66.90\% \\
\gemadv & 72.00\% & 0.55 & 0.93 & 0.69 & 77.89\% & 60.21\% \\
\bottomrule
\end{tabular}
\caption{Performance of different models on the Step Order Prediction task when also explaining its judgment.}
\label{tab:binary_explain}
\end{table*}
